BigRoots: An Effective Approach for Root-cause Analysis of Stragglers in Big Data System

Stragglers are commonly believed to have a great impact on the performance of big data system. However, the reason to cause straggler is complicated. Previous works mostly focus on straggler detection, schedule level optimization and coarse-grained cause analysis. These methods cannot provide valuable insights to help users optimize their programs. In this paper, we propose BigRoots, a general method incorporating both framework and system features for root-cause analysis of stragglers in big data system. BigRoots considers features from big data framework such as shuffle read/write bytes and JVM garbage collection time, as well as system resource utilization such as CPU, I/O and network, which is able to detect both internal and external root causes of stragglers. We verify BigRoots by injecting high resource utilization across different system components and perform case studies to analyze different workloads in Hibench. The experimental results demonstrate that BigRoots is effective to identify the root cause of stragglers and provide useful guidance for performance optimization.

==> bibliography.tex <==
\begin{thebibliography}{1}

\bibitem{mapreduce}J.Dean, S. Ghemawat, "MapReduce: Simplified Data Processing on Large Clusters." Communications of the ACM, pp. 107-113, 2008.
\bibitem{dryad}M. Isard, M. Mihai, Y. Yu A. Birrell, D. Fetterly. "Dryad: Distributed Data-parallel Programs from Seq1uential Building Blocks." ACM SIGOPS Operating Systems Review, vol. 41, no. 3, pp. 59-72. 2007.
\bibitem{spark}M. Zaharia, M. Chowdhury, M. J. Franklin, S. Shenker, I. Stoica. "Spark: Cluster Computing with Working Sets." USENIX conference on Hot Topics in Cloud Computing, vol. 10, pp. 10, 2010.
\bibitem{straggler_impact}P. Garraghan, X. Ouyang, R. Yang, D. McKee, and J. Xu, "Straggler root-cause and impact analysis for massivescale virtualized cloud datacenters.", IEEE Transactions on Services Computing, vol. PP, no. 99, pp. 1¡§C1, 2017.
\bibitem{straggler_google}J. Dean, L. A. Barroso. "The Tail at Scale." Communications of the ACM 56, no. 2, pp. 74-80, 2013.
\bibitem{straggler_bing}G. Ananthanarayanan, S. Kandula, A. G. Greenberg, I. Stoica, Y. Lu, B. Saha, and E. Harris. "Reining in the Outliers in Map-Reduce Clusters using Mantri." OSDI, vol. 10, no. 1, pp. 24, 2010.
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TODO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{google_estimation}J. Dean and S. Ghemawat. MapReduce: Simplified Data Processing on Large Clusters. In Communications of the ACM, 51 (1): 107-113, 2008.
\bibitem{late}Zaharia, Matei, et al. "Improving MapReduce performance in heterogeneous environments." Usenix Conference on Operating Systems Design and Implementation USENIX Association, 2008:29-42.
\bibitem{mantri}Ganesh Ananthanarayanan, et al. "Reining in the Outliers in Map-Reduce Clusters using Mantri. " Usenix Symposium on Operating Systems Design and Implementation, OSDI 2010, October 4-6, 2010, Vancouver, Bc, Canada, Proceedings DBLP, 2010:265-278.
\bibitem{dolly}Ananthanarayanan, Ganesh, et al. "Effective straggler mitigation: attack of the clones." Usenix Conference on Networked Systems Design and Implementation USENIX Association, 2013:185-198.
\bibitem{speculation_waste}E. Bortnikov, A. Frank, E. Hillel, S. Rao. "Predicting Execution Bottlenecks in Map-reduce Clusters." USENIX conference on Hot
Topics in Cloud Computing, pp. 18-18, 2012
\bibitem{cause_simple}Ouyang, Xue, et al. "Reducing Late-Timing Failure at Scale: Straggler Root-Cause Analysis in Cloud Datacenters." The, Ieee/ifip International Conference on Dependable Systems and Networks IEEE, 2016.
\bibitem{performance_instrument}Ousterhout, Kay, et al. "Making sense of performance in data analytics frameworks." Usenix Conference on Networked Systems Design and Implementation USENIX Association, 2015:293-307.
\bibitem{hibench}S. Huang, J. Huang, J. Dai, T. Xie, and B. Huang, "The hibench benchmark suite: Characterization of the mapreduce-based data analysis", IEEE International Conference on Data Engineering Workshops, 2010, pp. 41¡§C51.
\bibitem{tsar}Tsar tools, available: https://github.com/alibaba/tsar/
\bibitem{nagios}Nagios, available: https://www.nagios.org/
\bibitem{web_bayesian}Xiaohui Gu and Haixun Wang. Online anomaly prediction for robust cluster systems. In IEEE 25th International Conference on Data Engineering, 2009. ICDE¡¯09, pages 1000¨C1011. IEEE, 2009.
\bibitem{web_unsupervised}Daniel Joseph Dean, Hiep Nguyen, and Xiaohui Gu. Ubl: unsupervised behavior learning for predicting performance anomalies in virtualized cloud systems. In Proceedings of the 9th international conference on Autonomic computing, pages 191¨C200. ACM, 2012.
\bibitem{web_rootcause}Jayathilaka, Hiranya, C. Krintz, and R. Wolski. "Performance Monitoring and Root Cause Analysis for Cloud-hosted Web Applications." International Conference on World Wide Web International World Wide Web Conferences Steering Committee, 2017:469-478.
\bibitem{web_anomaly}Magalhaes, Joao Paulo, and L. M. Silva. "Detection of Performance Anomalies in Web-Based Applications." Ninth IEEE International Symposium on Network Computing and Applications IEEE Computer Society, 2010:60-67.
\bibitem{web_correlation}Joao Paulo Magalhaes and Luis Moura Silva. Root-cause analysis of performance anomalies in web-based applications. In Proceedings of the 2011 ACM Symposium on Applied Computing, pages 209¨C216. ACM, 2011.
\bibitem{icdcs_utilization_monitor}Lai, Chien An, et al. "milliScope: A Fine-Grained Monitoring Framework for Performance Debugging of n-Tier Web Services." IEEE, International Conference on Distributed Computing Systems IEEE, 2017:92-102.
\bibitem{icdcs_holistic_analysis}Arefin, Ahsan, et al. "Diagnosing Data Center Behavior Flow by Flow." IEEE, International Conference on Distributed Computing Systems IEEE Computer Society, 2013:11-20.
%\bibitem{icpp_mistake}Pedersen, Jan B, et al. "Error Classifications for Parallel Message Passing Programs: A Case Study." Parallel and Distributed Processing Techniques and Applications 2012.
%\bibitem{icpp_casita}Schmitt, Felix, J. Stolle, and R. Dietrich. "CASITA: A Tool for Identifying Critical Optimization Targets in Distributed Heterogeneous Applications." International Conference on Parallel Processing Workshops IEEE, 2014:186-195.
%\bibitem{icpp_parallel_rootcause}Bohme, David, et al. "Identifying the Root Causes of Wait States in Large-Scale Parallel Applications." International Conference on Parallel Processing IEEE, 2010:11.
%\bibitem{wait_meira}Meira Jr, Wagner, Thomas J. LeBlanc, and Alexandros Poulos. "Waiting time analysis and performance visualization in Carnival." Proceedings of the SIGMETRICS symposium on Parallel and distributed tools. ACM, 1996.
%\bibitem{wait_meira2}Meira Jr, Wagner, Thomas J. LeBlanc, and Virg¡§alio AF Almeida. "Using cause-effect analysis to understand the performance of distributed programs." Proceedings of the SIGMETRICS symposium on Parallel and distributed tools. ACM, 1998.
%\bibitem{wait_jafri} Jafri, Hassan M. ?¡ãMeasuring Causal Propagation of Overhead of Inefficiencies in Parallel Applications?¡À. In Proc. of the 19th IASTED International Conference on Parallel and Distributed Computing and Systems. Cambridge, MA, USA, 237-243.
%\bibitem{wait_morajko} Oleg Morajko, Anna Morajko, Tomas Margalef, and Emilio Luque. 2008. On-Line Performance Modeling for MPI Applications. In Proc. of the 14th Euro-Par Conference (Las Palmas de Gran Canaria, Spain) (Lecture Notes in Computer Science), Vol. 5168. Springer, 68-77.
%\bibitem{wait_martin} Martin Schulz, Greg Bronevetsky, and Bronis R. de Supinski. 2008. On the Performance of Transparent MPI Piggyback Messages. In Proc. 15th European PVM/MPI Users' Group Meeting (Dublin, Ireland) (Lecture Notes in Computer Science), Vol. 5205. Springer, 194-201.
%\bibitem{wait_szebenyi} Zoltan Szebenyi, Brian J. N. Wylie, and Felix Wolf. 2008. Scalasca Parallel Performance Analyses of SPEC MPI2007 Applications. In Proc. of the 1st SPEC Int'l Performance Evaluation Workshop (SIPEW, Darmstadt, Germany) (Lecture Notes in Computer Science), Vol. 5119. Springer, 99-123.
\bibitem{hedera}Al-Fares, Mohammad, et al. "Hedera: dynamic flow scheduling for data center networks." Usenix Symposium on Networked Systems Design and Implementation, NSDI 2010, April 28-30, 2010, San Jose, Ca, Usa DBLP, 2010:281-296.
\bibitem{tachyon}Li, et al. "Tachyon: Reliable, Memory Speed Storage for Cluster Computing Frameworks." (2014):1-15.
\bibitem{google_trace_analysis}Reiss, Charles, et al. "Heterogeneity and dynamicity of clouds at scale:Google trace analysis." ACM Symposium on Cloud Computing ACM, 2012:1-13.
\bibitem{titan}Shi, Juwei, et al. "Clash of the titans: MapReduce vs. Spark for large scale data analytics." Proceedings of the Vldb Endowment 8.13(2015):2110-2121.
\bibitem{skewtune}Kwon, Yong Chul, et al. "SkewTune:mitigating skew in mapreduce applications." ACM SIGMOD International Conference on Management of Data ACM, 2012:25-36.
\end{thebibliography}

